groupShapley: Efficient prediction explanation with Shapley values for feature groups

Shapley values has established itself as one of the most appropriate and theoretically sound frameworks for explaining predictions from complex machine learning models. The popularity of Shapley values in the explanation setting is probably due to its unique theoretical properties. The main drawback with Shapley values, however, is that its computational complexity grows exponentially in the number of input features, making it unfeasible in many real world situations where there could be hundreds or thousands of features. Furthermore, with many (dependent) features, presenting/visualizing and interpreting the computed Shapley values also becomes challenging. The present paper introduces groupShapley: a conceptually simple approach for dealing with the aforementioned bottlenecks. The idea is to group the features, for example by type or dependence, and then compute and present Shapley values for these groups instead of for all individual features. Reducing hundreds or thousands of features to half a dozen or so, makes precise computations practically feasible and the presentation and knowledge extraction greatly simplified. We prove that under certain conditions, groupShapley is equivalent to summing the feature-wise Shapley values within each feature group. Moreover, we provide a simulation study exemplifying the differences when these conditions are not met. We illustrate the usability of the approach in a real world car insurance example, where groupShapley is used to provide simple and intuitive explanations.

==> Newcommands.tex <==


\newtheorem{thm}{Theorem}[section] 
\newtheorem{lem}[thm]{Lemma}
\newtheorem{ass}[thm]{Assertion}
\newtheorem{rem}{Remark}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{defn}[thm]{Definition}

\newtheorem{assump}[thm]{Assumption}



%%%%% New commands
\newcommand{\hatt}[1]{\widehat{#1}}
\newcommand{\mupm}{\widehat{\mu}_{{\rm{pm}}}}
\newcommand{\munp}{\widehat{\mu}_{{\rm{np}}}}
\newcommand{\para}{{\rm{pm}}}
\newcommand{\nonpara}{{\rm{np}}}
\newcommand{\tr}{{\rm{t}}}


\newcommand{\mupmi}[1]{\widehat{\mu}_{{\rm{pm}}^{(#1)}}}

\newcommand{\muhat}{\widehat{\mu}}
\newcommand{\varhat}{\widehat{{\rm{Var}}}}
\newcommand{\covhat}{\widehat{{\rm{Cov}}}}
\newcommand{\hn}{\bar{h}_n}
\newcommand{\rderiv}{\left(\frac{\partial r}{\partial \theta}(\hat{\theta})\right)}
\newcommand{\rderivt}{\left(\frac{\partial r}{\partial \theta}(\hat{\theta})\right)^t}
\newcommand{\dd}{\, \mathrm{d}}

\newcommand{\convp}{\stackrel{P}{\rightarrow}}
\newcommand{\convl}{\stackrel{L}{\rightarrow}}
\newcommand{\convas}{\stackrel{a.s.}{\rightarrow}}

\renewcommand{\Pr}[1]{\text{Pr}\left( #1 \right)}

%\newcommand{\infl}[3]{\mathcal{I}_{#1}(#2;#3)}
%\newcommand{\inflbar}[2]{\overline{\mathcal{I}}_{#1,n}(#2)}
\newcommand{\infl}[3]{{\rm{IF}}_{#1}(#2;#3)}
\newcommand{\inflbar}[2]{\overline{{\rm{IF}}}_{#1,n}(#2)}

%\newcommand{\empinfl}[2]{d_{#1,#2}}
\newcommand{\empinfl}[2]{\infl{\mu}{Y_i}{\Gnhat}}

\newcommand{\ind}[1]{\mathbf{I} \left\{ #1 \right\}}
\newcommand{\indtwo}[2]{\mathbf{1}_{\left\{ #2 \right\}}{\left(#1\right)}}


\newcommand{\E}[2]{\text{E}_{#1}[#2]}
\newcommand{\Var}[2]{{\rm{Var}}_{#1}(#2)}
\newcommand{\Cov}[2]{{\rm{Cov}}_{#1}(#2)}

\newcommand{\ecdf}[1]{\widehat{{#1}_n}}

\newcommand{\npvar}{\nu}
\newcommand{\npvarhat}{\widehat{\nu}}

\newcommand{\Gnhat}{\widehat{G}_n}
\newcommand{\muGnhat}{\mu(\widehat{G}_n)}

\newcommand{\mutrue}{\mu_{\rm{true}}}
\newcommand{\mupmlf}{\mu_{0,\rm{pm}}}

\newcommand{\argmax}[1]{\underset{#1}{\operatorname{argmax}}\:}
\newcommand{\MLtheta}{\widehat{\theta}_n}

\newcommand{\biaspm}{{\rm{bias}}_{\rm{pm}}}
\newcommand{\biaspmhat}{\widehat{\rm{bias}}_{\rm{pm}}}
\newcommand{\bhat}{\widehat{b}}
\newcommand{\sqbiaspmhatone}{\widehat{{\rm{bias}}^2}^*_{\rm{pm}}}
\newcommand{\sqbiaspmhat}{\widehat{{\rm{bias}}^2}_{\rm{pm}}}

\newcommand{\biasnp}{{\rm{bias}}_{\rm{np}}}
\newcommand{\biasnphat}{\widehat{\rm{bias}}_{\rm{np}}}
\newcommand{\sqbiasnphat}{\widehat{\rm{bias}^2}_{\rm{np}}}

\newcommand{\Vpm}{V_{\rm{pm}}}
\newcommand{\Vnp}{V_{\rm{np}}}
\newcommand{\Vpmnp}{V_{\rm{pm,np}}}
\newcommand{\Vb}{V_{\rm{b}}}
\newcommand{\N}{{\rm{N}}}


\newcommand{\Vnpstar}{V^*_{\rm{np}}}

\newcommand{\Vhatnp}{\widehat{V}_{\rm{np}}}
\newcommand{\Vhatpm}{\widehat{V}_{\rm{pm}}}
\newcommand{\Vhatpmnp}{\widehat{V}_{\rm{pm,np}}}
\newcommand{\Vhatb}{\widehat{V}_{\rm{b}}}

\newcommand{\muFderiv}[1]{\frac{\partial \mu_F}{\partial \theta}\bigg|_{#1}}


\newcommand{\mockalph}[1]{}




